Does Vec2Text Pose a New Corpus Poisoning Threat?

The emergence of Vec2Text -- a method for text embedding inversion -- has raised serious privacy concerns for dense retrieval systems which use text embeddings. This threat comes from the ability for an attacker with access to embeddings to reconstruct the original text. In this paper, we take a new look at Vec2Text and investigate how much of a threat it poses to the different attacks of corpus poisoning, whereby an attacker injects adversarial passages into a retrieval corpus with the intention of misleading dense retrievers. Theoretically, Vec2Text is far more dangerous than previous attack methods because it does not need access to the embedding model's weights and it can efficiently generate many adversarial passages. We show that under certain conditions, corpus poisoning with Vec2Text can pose a serious threat to dense retriever system integrity and user experience by injecting adversarial passaged into top ranked positions. Code and data are made available at https://github.com/ielab/vec2text-corpus-poisoning

==> sections/experiments.tex <==
\begin{table*}\centering
\captionsetup{skip=5pt}
	\caption{Reproduction of the DPR~\cite{karpukhin-etal-2020-dense} embedding models with different distance metrics and pooling functions. "cls" indicates the utilization of the CLS token embedding as the representation, while "mean" indicates the use of mean pooling, aggregating all token embeddings to generate the final text embedding. "dot" indicates the dot product distance metric and "cos" indicates the cosine similarity distance metric. There is no statistically significant difference observed in terms of retrieval effectiveness.}
	\label{tab:dpr}
	%	\resizebox{0.9\textwidth}{!}{
		\begin{tabular}{@{}lllrrrrrrrr@{}}\toprule
		\multicolumn{3}{c}{\bf Embedding Models} & \multicolumn{4}{c}{\bf Retrieval effectiveness} & \multicolumn{4}{c}{\bf Reconstructibility} \\
		\cmidrule(lr){4-7} \cmidrule(l){8-11}
		Label & Metric & Representation
			&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
			a. DPR\_cls\_dot & Dot-product & CLS token & 0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
			b. DPR\_cls\_cos & Cosine similarity & CLS token &0.748 &0.799 &0.863 &0.914 &71.834 &0.879 &0.345 &0.975 \\
			c. DPR\_mean\_cos & Cosine similarity & Mean pooling &0.745 &0.802 &0.866 &0.916 &81.918 &0.924 &0.480 &0.988 \\
			\bottomrule
		\end{tabular}
		%	}
\end{table*}

\section{Understanding what impacts Vec2Text effectiveness}
In the previous sections, we successfully reproduced Vec2Text with the GTR-base embedding model and finalized the experimental environment. In this section, our goal is to understand how various strategies implemented by different embedding models impact retrieval effectiveness and Vec2Text reconstructibility. To achieve this, we re-train Vec2Text with respect to the target embedding models. Each of the embedding models represents different choices in terms of distance metric, pre-training strategy, etc. When re-training, we used the same Vec2Text parameters reported above.

%against target embedding models that were trained with different strategies, using the exact same parameters.

To maintain control over experimental parameters and prevent results from being influenced by factors such as different datasets and training parameters, we independently train the embedding models ourselves. This is done with the same experimental settings but utilizing different training or inference strategies. Specifically, we start by reproducing the DPR embedding model~\cite{karpukhin-etal-2020-dense}, following the training parameters outlined in the DPR paper and employing the Tevatron dense retriever training toolkit~\cite{gao2023tevatron} to train the DPR model on the NQ dataset, the same dataset used to train Vec2Text. After reproducing the DPR retrieval results, we then apply the same dense retriever training hyperparameters (e.g., batch size, learning rate, and number of hard negatives) to train other DPR variations with distinct training strategies, as detailed in the next subsections.


\subsection{Distance Metric and Pooling Method}
In Table~\ref{tab:dpr}, we examine the impact of different distance metrics, namely dot product (dot) or cosine similarity (cos), used for training and inference in DPR models. Additionally, we investigate the pooling method employed to construct a single embedding for each input text, specifically, CLS token embedding (cls) or mean pooling of all token embeddings (mean).

The \textit{DRP\_cls\_dot} represents our reproduction of the original DPR embedding model, utilizing CLS token embedding to represent the entire text and employing the dot product during training. We achieved very similar top-k retrieval effectiveness as reported in the original DPR paper, indicating successful reproduction of DPR. It is worth noting that our trained \textit{DRP\_cls\_dot} exhibits higher retrieval effectiveness than GTR-base embedding models presented in Table~\ref{tab:reproduce}, possibly due to our DPR training and testing data originating from the same data distribution, while GTR-base has training data from other domains.

However, concerning Vec2Text reconstructibility, we observe that Vec2Text trained with the \textit{DRP\_cls\_dot} embedding model yields much lower reconstructibility compared to GTR-base embedding models. This suggests that the embeddings provided by \textit{DRP\_cls\_dot} contain less information for Vec2Text to reconstruct the original text, indicating a potentially more secure embedding model than GTR-base.


We then proceeded to train two additional DPR variations, namely \textit{DRP\_cls\_cos}, which employs CLS token embedding and cosine similarity, and \textit{DRP\_mean\_cos}, which utilizes mean pooling of all token embeddings with cosine similarity. There was no statistically significant differences in retrieval effectiveness for these settings.

Regarding reconstructibility, a comparison between \textit{DRP\_cls\_dot} and \textit{DRP\_cls\_cos} suggests that cosine similarity appears to enhance Vec2Text's exact matching score. However, when comparing \textit{DRP\_cls\_cos} and \textit{DRP\_mean\_cos}, the reconstructibility of Vec2Text significantly increases. This surprising result suggests that mean pooling is a key factor for Vec2Text reconstructibility but does not necessarily contribute to improved retrieval effectiveness. We suspect that this might be due to mean pooling explicitly gathering all the token information into the embedding, whereas the CLS token embedding only implicitly learns the text information during DR training, making it less helpful for Vec2Text training.
Consequently, practitioners in the field of DR should carefully consider avoiding the use of mean pooling to enhance the security of the embedding model against Vec2Text attacks.

It is worth noting that the GTR-base model exclusively employs mean pooling and cosine similarity. This may explain why Vec2Text achieves high reconstructibility scores when trained with GTR-base embedding models.


\begin{table*}[!htp]\centering
\captionsetup{skip=5pt}
	\caption{Zero-shot retrieval and bottlenecked pre-training results. 
		Subscripts denote statistically significantly better retrieval effectiveness with a T-test ($p < 0.01$). Results show that even zero-shot retrievers are at risk to Vec2Text reconstruction. Bottleneck pre-training proved useful at improve retrieval effectiveness but greatly increased risk of reconstructibility.}
	\label{tab:zeroshot}
	%	\resizebox{0.9\textwidth}{!}{
		\begin{tabular}{@{}llllllllll@{}}\toprule
			\multicolumn{2}{c}{\bf Embedding Models}&\multicolumn{4}{c}{\bf Retrieval effectiveness} & \multicolumn{4}{c}{\bf Reconstructibility} \\
			\cmidrule(lr){3-6}\cmidrule(l){7-10}
			Label & Setting& top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
			a. BERT\_cls\_dot & Zero-shot & 0.101 & 0.153& 0.288 &0.467 & 37.034& 0.671& 0.042& 0.968 \\
			b. BERT\_mean\_cos & Zero-shot &  0.283$^{a}$& 0.358$^{a}$& 0.520$^{a}$ & 0.715$^{a}$ & 80.057&0.914 &0.414 & 0.984\\
			c. SimLM\_cls\_dot & Bottleneck + Zero-shot  & 0.304$^{ab}$  & 0.378$^{a}$ & 0.546$^{ab}$  & 0.720$^{a}$  & 94.560& 0.974& 0.677& 0.999 \\\hline
			d. SimLM\_cls\_dot\_finetuned & Bottleneck + Fine-tuned & 0.750$^{abc}$ & 0.805$^{abc}$& 0.874$^{abc}$ & 0.919$^{abc}$ & 94.845& 0.975& 0.661& 0.997\\
			\bottomrule
		\end{tabular}
		%	}
\end{table*}




\subsection{Zero-shot Regime and Bottleneck Pre-training}
In the previous section, we delved into fine-tuned DPR embedding models. In this section, we further explore zero-shot dense retriever with pre-trained, zero-shot embedding models. The aim is to investigate if the DR fine-tuning (done in the previous sections) itself leads to vulnerability from Vec2Text. Additionally, we explore embedding models that leverage bottleneck pre-training designed to enhance the CLS token embedding. The results are presented in Table~\ref{tab:zeroshot}.

\textit{BERT\_cls\_dot} and \textit{BERT\_mean\_cos} use the same backbone pre-trained embedding model (BERT~\cite{kenton2019bert}) and perform the exact same inference as \textit{DRP\_cls\_dot} and \textit{DRP\_mean\_cos} but without DPR training; they represent zero-shot retrievers. Their zero-shot retrieval effectiveness is significantly worse than fine-tuned DPR models (as might be expected for a zero-shot dense retriever). Mean pooling with cosine similarity exhibits higher zero-shot retrieval effectiveness than dot product with CLS token embeddings but still well below the trained DPR models from the previous section.

Now considering reconstructibility, \textit{BERT\_cls\_dot} is much less vulnerable than than \textit{DRP\_cls\_dot}.
This suggests that DR fine-tuning injects information that could aid Vec2Text in reconstruction from the CLS token embedding. In contrast, \textit{BERT\_mean\_cos} already demonstrates strong Vec2Text reconstructibility, further confirming that mean pooling with cosine similarity is potentially problematic --- even for the zero-shot setting.


We then tested the SimLM~\cite{wang-etal-2023-simlm} embedding model, which leverages a bottlenecked pre-training approach~\cite{gao-callan-2021-condenser,lu-etal-2021-less,liu2022retromae,shen2022lexmae,chuang2022diffcse,wu2022contextual,zhuang2023toroder}. Bottlenecked pre-training is a task designed to enhance the CLS token embedding. This is achieved by taking the embedding model's outputted CLS token embedding and inputting it into a weaker decoder model. The pre-training objective is to enable the decoder model to perform the MASK language modelling task or, in the case of SimLM, the ELECTRA pre-training task~\cite{clark2019electra}. Consequently, the model must learn to inject useful information into the CLS token embedding to assist the decoder in completing the task. In fact, this pre-training approach closely resembles Vec2Text training itsself, as both involve a generator that takes an embedding as input and attempts to reconstruct a piece of text. Previous studies on bottlenecked pre-training have shown improvements in DR retrieval effectiveness. However, we suspect that this pre-training approach may make the embedding particularly vulnerable to Vec2Text, raising potential privacy concerns.

Our results confirmed our hypothesis: \textit{SimLM\_cls\_dot} with additional bottlenecked pre-training on the NQ datasets\footnote{\url{https://huggingface.co/intfloat/simlm-base-wiki100w}}, demonstrated higher zero-shot retrieval effectiveness than \textit{BERT\_mean\_cos}, indicating that bottlenecked pre-training injected useful information into the CLS token that can aid in retrieval. However, the enhanced CLS token embedding proved highly vulnerable to Vec2Text. The BLEU, TF1, and COS scores were even higher than those achieved by Vec2Text trained with correct GTR-base embeddings. We conducted further tests by using SimLM as the backbone model instead of BERT to train a DPR model with the same training parameters as \textit{DPR\_cls\_dot}. The results are outlined in the row labeled \textit{SimLM\_cls\_dot\_finetuned}. Indeed, the use of SimLM further improved DPR retrieval effectiveness and also achieved very high reconstructibility. We conclude that practitioners should carefully consider the privacy implications of bottleneck pre-training before incorporating this approach.

\begin{table*}\centering
\captionsetup{skip=5pt}
	\caption{Impact of embedding dimension and quantization. Both dimension reduction and product quantization prove to be simple and effective methods to mitigate Vec2Text reconstruction, without comprising retrieval effectiveness. There is no statistically significant difference observed in terms of retrieval effectiveness.}\label{tab:dim}
		\addtolength{\tabcolsep}{-0.2em}
%	\resizebox{1\textwidth}{!}{
		\begin{tabular}{@{}lrlrrrrrrrrr@{}}\toprule
			\multicolumn{3}{c}{\bf Embedding Models}& \bf Index size &\multicolumn{4}{c}{\bf Retrieval effectiveness} &\multicolumn{4}{c}{\bf Reconstructibility} \\
			\cmidrule(r){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-8}\cmidrule(l){9-12}
			Label & Dim. & Quantization & & top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
			a. DPR\_cls\_dot (768) & 768 & None &61GB &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
			b. DPR\_cls\_dot (256) & 256 & None &21GB &0.731 &0.784 &0.855 &0.910 &25.060 &0.565 &0.035 &0.881 \\
			c. DPR\_cls\_dot (PQ\_768) & 768 & Product &16GB &0.749 &0.801 &0.862 &0.914 &1.916 &0.146 &0.000 &0.748 \\
			d. DPR\_cls\_dot (PQ\_256) & 256 & Product &5GB &0.740 &0.796 &0.864 &0.912 &2.305 &0.159 &0.000 &0.767 \\
			\bottomrule
		\end{tabular}
%	}
\end{table*}

\subsection{Embedding Dimensionality \& Quantization}
Next, we explore how embedding dimensionality and quantization, popular methods for reducing DR index size and improving retrieval efficiency, impact retrieval effectiveness and Vec2Text reconstructability.

Regarding embedding dimensionality, we trained another DPR model with the exact settings as \textit{DPR\_cls\_dot}, but adding a dense pooling layer on top to reduce the embedding dimension from 768 to 256. This variant is labeled as \textit{DPR\_cls\_dot (256)}. For embedding quantization, we applied product quantization (PQ)~\cite{jegou2010product} to \textit{DPR\_cls\_dot}. We experimented with two settings: one with the number of sub-vectors set to 768 and another with 256. The number of bits per sub-vector for both settings is set to 8 in both cases, resulting in embedding dimensions of 768 and 256. We label them \textit{DPR\_cls\_dot (PQ\_768)} and \textit{DPR\_cls\_dot (PQ\_256)} respectively.

The results presented in Table~\ref{tab:dim} indicate that dimensionality reduction and product quantization can significantly reduce the dense vector index sizes, as expected. Product quantization demonstrates robust retrieval effectiveness; when the sub-vector is set to 768, there is no decrease in top-k accuracy, and only a slight decrease in retrieval effectiveness when further reducing the dimensionality to 256. These findings align with previous studies~\cite{ma-etal-2021-simple}.

On the other hand, simply reducing the embedding dimension by adding a dense pooling layer can considerably decrease Vec2Text reconstructibility, albeit at the cost of hurting retrieval effectiveness. PQ once again demonstrates superior privacy protection ability. Both settings of PQ we considered completely mitigate Vec2Text reconstructibility. Notably, this is achieved without compromising retrieval effectiveness, and the index size is significantly reduced. Hence, we conclude that product quantization is a simple and effective method for protecting embeddings from attacks by Vec2Text.




==> sections/mitigation.tex <==
\begin{figure}[h!]

  \includegraphics[width=.75\columnwidth]{figures/noise_plot.pdf}
  \caption{Impact on retrieval effectiveness and reconstructibility of different amounts of noise injection with different retrieval models. Larger $\lambda$ signifies more noise injection.}
  	\label{fig:noise_plot}
\end{figure}


\begin{table*}[!htp]\centering
\captionsetup{skip=5pt}
	\caption{Impact of adding noise and customized embedding transformation. Noise injection was an effective reconstruction mitigation strategy. The proposed vector transformation mitigation strategy is easily applied and guaranteed to maintain retrieval effective while completely degrading reconstructibility. There is no statistically significant difference observed in terms of retrieval effectiveness.}\label{tab:tranformation}
%	\resizebox{0.9\textwidth}{!}{
		\begin{tabular}{@{}llrrrrrrrr@{}}\toprule
			\multicolumn{2}{c}{\bf Embedding Models}&\multicolumn{4}{c}{\bf Retrieval effectiveness} &\multicolumn{4}{c}{\bf Reconstructibility} \\
			\cmidrule(r){1-2} \cmidrule(lr){3-6}\cmidrule(l){7-10}
			Label & Mitigation & top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
			a. DPR\_cls\_dot & None &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
			b. DPR\_cls\_dot\_noise & Noise injection &0.730 &0.790 &0.856 &0.911 &10.022 &0.415 &0.000 &0.823 \\
			c. DPR\_cls\_dot\_transform & Vector transformation &0.748 &0.800 &0.863 &0.914 &1.178 &0.065 &0.000 &0.443 \\
			\bottomrule
		\end{tabular}
%	}
\end{table*}


\begin{table*}[!htp]\centering
\captionsetup{skip=5pt}
	\caption{Results of adding noise during Text2Text training. The target embedding model is $DPR\_cls\_dot$. Noise injection proved to be an effective mitigation strategy even when Vec2Text is actually trained with noisy embeddings.}\label{tab:noise_train}
		\begin{tabular}{@{}llrrrrrrrr@{}}\toprule
			\multicolumn{2}{@{}c}{\bf Vec2Text Models} & \multicolumn{8}{c}{\bf Reconstructibility}\\
			& & \multicolumn{4}{c}{On original embeddings} & \multicolumn{4}{c}{On noisy embeddings} \\ 
			\cmidrule(r){1-2} \cmidrule(lr){3-6}\cmidrule(l){7-10}
			Label & Trained on &bleu &tf1 &exact &cos &bleu &tf1 &exact &cos \\\midrule
			Vec2Text & Original embeddings &70.735 &0.875 &0.319 &0.985 &10.022 &0.415 &0.000 &0.823 \\
			Vec2Text\_noise & Noisy embeddings &29.264 &0.635 &0.012 &0.966 &17.417 &0.504 &0.005 &0.882 \\
			\bottomrule
		\end{tabular}
\end{table*}



\section{Mitigation Strategies}
In the previous sections, we explored how different DR training and inference strategies trade-off retrieval effectiveness and embedding privacy protection. In this section, we evaluate methods that proactively protect against the Vec2Text attacks.

\subsection{Noise Injection}
In the original Vec2Text paper, \citeauthor{morris-etal-2023-text} explored a basic mitigation strategy of adding Gaussian noise directly to each embedding:
\begin{equation}
	\phi_{noisy}(x) = \phi(x) + \lambda \cdot \epsilon, \epsilon \sim  \mathcal{N}(0, 1),
\end{equation}
where $\phi(x)$ is the embedding for a given input text $x$, $\epsilon$ is the noise vector whose elements are sampled from a Gaussian distribution, and $\lambda$ is a hyperparameter controlling the amount of injected noise.  \citeauthor{morris-etal-2023-text} showed that setting $\lambda = 0.1$ completely prevents reconstructibility for the GTR-base embedding model, but it also has a major negative impact on retrieval effectiveness.



%would destroy both retrieval effectiveness and Vec2Text reconstructibility for the GTR-base embedding model (with incorrect embeddings).

Here, we reproduce the noise injection mitigation strategy on our trained $DPR\-\_cls\_dot$ embedding model, labeled as $DPR\_cls\_dot\_noise$ in Table~\ref{tab:tranformation}. Our results show partially different outcomes: setting $\lambda = 0.1$ did indeed prevent Vec2Text reconstructibility but only slightly impacted retrieval effectiveness. 
This may be due to the sensitivity of the specific embedding models to the amount of noise (as controlled by $\lambda$). To better understand this we completed a sweep of $\lambda = [0.001, 0.01, 0.1, 1.0]$ for DPR, GTR and GTR with corrected embeddings; this is shown in Figure~\ref{fig:noise_plot}. We observe that DPR requires more noise to see an effect: both in terms of retrieval effectiveness deterioration, and reconstructibility robustness. We hypothesise that this is due to the different distance metric used by the two methods (GTR uses cosine, while DPR here uses dot product).
Overall, adding noise remains a desirable mitigation strategy but correct parameter setting is critical. However, the correct setting of the noise parameter appears to be dependent on the specific embedding model used. In the next section we propose a new mitigation strategy that does not have this drawback. 


A question still remains, though, of whether adding noise was an effective mitigation strategy if Vec2Text was actually trained using these noisy vectors. 
To investigate this, we re-trained a Vec2Text model while adding the same Gaussian noise to the input embeddings. The results are presented in Table~\ref{tab:noise_train}. Our findings demonstrate that adding noise to Vec2Text training reduces reconstructibility on original embeddings. While it does make Vec2Text more robust to noisy embeddings, the level of reconstructibility remains very low. Thus, we conclude that adding noise to Vec2Text training does not make the noise-adding defence vulnerable.


\subsection{Embedding Transformation}

Finally, we propose a new mitigation strategy that prevents reconstruction via Vec2Text but has the benefit of theoretically guaranteeing no change in retrieval effectiveness and not requiring parameter tuning that is dependent on the embedding model used. 

Our idea is straightforward: we propose applying a simple transformation to all the embeddings, with a transform function customized and only visible to each user (similar to an API key) who sends text to the embedding model APIs (such as OpenAI users sending text to OpenAI APIs to obtain embeddings). Formally, we define the transformed embeddings as:
\begin{equation}
	\phi_{\text{transformed}}(x) = f(\phi(x)),
\end{equation}
where $f$ is a linear transformation function unique to each user. For example, in our experiments, we simply set $ f(\phi(x)) = -2.6 \cdot \phi(x)$ so all embeddings are adjusted by a constant value. The function (in our case the constant value) is kept secret and thus not known to a Vec2Text attacker. This means that attackers will obtain different embeddings from the API calls to train their Vec2Text model. Additionally, on the user side, since the same transformation function is applied to all embeddings retrieval will not be impacted. Users can still reverse engineer to get the original embeddings since the transformation function is visible to the user.

We present our empirical results in Table~\ref{tab:tranformation}, labeled with \textit{DPR\-\_cls\_dot\_transform} (row c.). Note that the retrieval effective is identical to that of \textit{DPR\-\_cls\_dot} (row a.), as guaranteed by the uniform transformation. At same time, reconstructibility is almost completely degraded so privacy is protected. We believe this simple strategy could be easily adopted by service providers like OpenAI or Cohere to offer their users the option to make their embeddings more secure.



==> sections/reproduction.tex <==
\section{Reproduction of vec2text}

\subsection{Experimental Methodology}

\begin{table*}[h]
\captionsetup{skip=5pt}
	\caption{Reproduction results of Vec2Text \cite{morris-etal-2023-text} comparing retrieval effectiveness and text reconstructibility. Bug fixed represents a correction to ensure Vec2Text uses the final dense pooling layer of GTR-base for output. Subscripts denote statistically significantly difference in retrieval effectiveness using a paired, two-tails t-test ($p < 0.01$).}\label{tab:reproduce}
		\begin{tabular}{@{}lllllllll@{}}
			\toprule
			\multirow{2}{*}{\bf Embedding Models}&\multicolumn{4}{c}{\bf Retrieval effectiveness} & \multicolumn{4}{c}{\bf Reconstructibility} \\
			\cmidrule(lr){2-5} \cmidrule(lr){6-9}
			&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
			a. GTR-base (original) &0.634 &0.711 &0.816 &0.893 &90.128 &0.970 &0.758 &0.990 \\
			b. GTR-base (reproduced \cite{morris-etal-2023-text}) &0.634 &0.711 &0.816 &0.893 &88.956 &0.971 &0.699 &0.996 \\
			c. GTR-base (bug fixed) &0.718$^{ab}$ &0.773$^{ab}$ &0.855$^{ab}$ &0.913$^{ab}$ &90.362 &0.970 &0.752 &0.998 \\ 
			\bottomrule
		\end{tabular}
\end{table*}

We begin by completing a full reproduction of Vec2Text. This is needed to ensure a fair comparison of the different embeddings models and settings with which we further study Vec2Text.

We use the official Vec2Text codebase\footnote{\url{https://github.com/jxmorris12/vec2text}} provided by the authors and adhere to the training parameters outlined in the original Vec2Text paper. Specifically, we train Vec2Text on documents from the Natural Question (NQ) dataset~\cite{kwiatkowski-etal-2019-natural}, setting the max sequence length to 32. The Adam optimizer is employed with a learning rate of $2 \times 10^{-4}$, incorporating warmup and linear decay. A batch size of 512 is utilized, and all models are trained on a single H100 GPU. The only deviation from the original setting is the number of training epochs. We note that the complete Vec2Text training pipeline is time-consuming. The authors reported in the paper that the full pipeline takes 2 days to train for 100 epochs with four A6000 GPUs. However, in our implementation using the provided code, the full pipeline takes approximately 10 days with a single H100 GPU. Given the extensive number of embedding models we plan to investigate and the limited computational resources at our disposal, we train for 50 epochs. This reduces the training time to around 5 days for each embedding model, making the process more feasible within our constraints. For the Vec2Text inference, we always use beam search with 50 steps and a beam width 4.

In addition to the variation in the number of epochs, we have identified a significant issue in the original experiment involving the training of Vec2Text for reconstructing text from the GTR-base embeddings. %\footnote{At times, we shall refer to this process as \textit{embedding inversion}.}. 
\citeauthor{morris-etal-2023-text} inadvertently used the last hidden layer outputs of the GTR-base model as the final text embeddings. However, it's crucial to note that GTR-base incorporates an additional dense pooling layer to project the last hidden layer outputs, a detail overlooked by the Vec2Text training code.
To address this issue, this section includes a re-training of Vec2Text with the correct GTR-base embeddings, and we compare the results with the original setting. This correction ensures a more accurate evaluation of Vec2Text's performance in inverting GTR-base embeddings.


Finally, to compare how different embedding models balance retrieval effectiveness and privacy preservation, we also measure the retrieval effectiveness of all considered embedding models. Following the original Vec2Text training setting, which involves training Vec2Text on documents from the NQ dataset, we adopt the \textit{top-k retrieval accuracy} evaluation setting from DPR~\cite{karpukhin-etal-2020-dense}, which measures the percentages of retrieved passages that contain a span that answers the
question (query). This evaluation is commonly employed in the literature for assessing retrieval effectiveness on the NQ dataset~\cite{gao-callan-2022-unsupervised, wang-etal-2023-simlm, qu-etal-2021-rocketqa, ma-etal-2021-simple, xiong2020approximate}. We use the official NQ test queries and Pyserini~\cite{jimmy2021pyserini} IR toolkit for this evaluation.

To evaluate reconstructibility, i.e. the ability to recover the original text from its embedding, we adopt the same measures used by \citet{morris-etal-2023-text}: 
\begin{itemize}
	\item BLEU score~\cite{Papineni2002bleu}, a metric capturing n-gram similarities between the true and reconstructed text;
	\item Token F1, representing the multi-class F1 score between the predicted and true token sets;
	\item Exact-match, indicating the percentage of reconstructed outputs perfectly matching the ground truth;
	\item Cosine similarity, measuring the similarity between the true embedding and the embedding of the reconstructed text.
\end{itemize}
 \noindent We randomly sample 1,000 passages from a held-out set of NQ training data for this evaluation\footnote{From their code, we understood that also \citeauthor{morris-etal-2023-text} performed sampling; while they do not mention how many passages they sampled, the default value in their code is 1,000 and so we adopted that value.}.


\subsection{Reproduction Results}

Table~\ref{tab:reproduce} shows Vec2Text reproduction results. The first row in the table shows the results obtained using the Vec2Text model checkpoint provided by the authors, which was trained with incorrect GTR-base embeddings. Despite the incorrect embeddings, the results indicate that it still performs well for retrieval, yielding reasonable top-k retrieval accuracy. Additionally, Vec2Text demonstrates robust reconstructibility. It is noteworthy that these outcomes are achieved with the incorrect GTR-base embeddings (without the dense pooling layer), suggesting that the last hidden layer of GTR-base already contains sufficient information for Vec2Text to effectively reconstruct the original input text.

The second row in the table shows the results obtained by our reproduced Vec2Text model with incorrect GTR-base embeddings (i.e., trying to exactly reproduce the original Vec2Text results). The only difference from the first row is the number of epochs; our reproduction uses half the number of epochs (50 epochs) compared to the original checkpoint (100 epochs). Since our goal is to replicate the original Vec2Text results, we also utilize the incorrect GTR-base embeddings, resulting in exactly the same retrieval effectiveness to the original setting. Regarding Vec2Text reconstructibility, our reproduced checkpoint only shows a slight decrease in the exact match score but achieves very close scores on other evaluation metrics. These results suggest that Vec2Text almost converges with half of the epochs than those used by \citeauthor{morris-etal-2023-text}, and the only notable improvement with longer training is in exact reconstruction. From here we only consider Vec2Text models trained on 50 epochs, noting their results are likely similar to those obtained if 100 epochs were used.

Finally, in the last row, we present our results using the correct GTR-base embeddings for retrieval and training Vec2Text with 50 epochs. Our findings emphasize the significance of using the correct embedding for retrieval, as the top-k accuracy exhibits a substantial increase compared to that obtained with incorrect embeddings. On the other hand, we achieve comparable Vec2Text reconstructibility with the original checkpoint, despite utilizing only half the training epochs. These results suggest that employing the correct outputs from the embedding model, rather than the intermediate layer outputs, may contribute to improved Vec2Text reconstruction.


==> sections/results.tex <==
\section{Results and Analysis}


\subsection{Reproducing with the correct GTR embedding}

\begin{table*}[!htp]\centering
	\caption{Reproduced results.}\label{tab: reproduce}
	\resizebox{0.9\textwidth}{!}{
	\begin{tabular}{l|llll | llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c|}{Retrieval effectiveness} & \multicolumn{4}{c}{Reconstructability} \\\cmidrule{2-9}
		 &top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		gtr-base (original) &0.634 &0.711 &0.816 &0.893 &90.128 &0.970 &0.758 &0.990 \\
		gtr-base (reproduced) &0.634 &0.711 &0.816 &0.893 &88.956 &0.971 &0.699 &0.996 \\
		gtr-base-st (bug fixed) &0.718 &0.773 &0.855 &0.913 &90.362 &0.970 &0.752 &0.998 \\ \hline
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cos &0.748 &0.799 &0.863 &0.914 &71.834 &0.879 &0.345 &0.975 \\
		DPR\_mean\_cos &0.745 &0.802 &0.866 &0.916 &81.918 &0.924 &0.480 &0.988 \\\hline
		BERT\_cls & 0.101 & 0.153& 0.288 &0.467 & 37.034& 0.671& 0.042& 0.968 \\
		BERT\_mean\_cos &  0.283& 0.358& 0.520 & 0.715 & 80.057&0.914 &0.414 & 0.984\\\hline
		SimLM-cls & 0.304  & 0.378& 0.546 & 0.720 & 94.560& 0.974& 0.677& 0.999 \\
		SimLM-cls-finetuned & 0.750 & 0.805& 0.874 & 0.919 & & & & \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Impact of distance metric and pooling}

\subsection{Impact of adding noise to the embedding}

\begin{table*}[!htp]\centering
	\caption{Impact of adding noise to the embedding}\label{tab:noise}
	\scriptsize
		\resizebox{1\textwidth}{!}{
	\begin{tabular}{l|llll|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c|}{Retrieval effectiveness} &\multicolumn{4}{c|}{Reconstruct effectiveness} &\multicolumn{4}{c}{Noise Reconstruct effectiveness} \\\cmidrule{2-13}
		&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 &10.022 &0.415 &0.000 &0.823 \\
		DPR\_cls\_noise &0.730 &0.790 &0.856 &0.911 &29.264 &0.635 &0.012 &0.966 &17.417 &0.504 &0.005 &0.882 \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Impact of embedding dimension and quantization}
\begin{table*}[!htp]\centering
	\caption{Impact of embedding dimension and quantization.}\label{tab: dim}
	\scriptsize
			\resizebox{1\textwidth}{!}{
	\begin{tabular}{l|l|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&Index size &\multicolumn{4}{c|}{Retrieval effectiveness} &\multicolumn{4}{c}{Reconstruct effectiveness} \\\cmidrule{2-10}
		&GB &top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls\_768 &61G &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cls\_256 &21G &0.731 &0.784 &0.855 &0.910 &25.060 &0.565 &0.035 &0.881 \\
		DPR\_cls\_PQ\_m768 &16G &0.749 &0.801 &0.862 &0.914 &1.916 &0.146 &0.000 &0.748 \\
		DPR\_cls\_PQ\_m256 &5.3G &0.740 &0.796 &0.864 &0.912 &2.305 &0.159 &0.000 &0.767 \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Customized embedding transformation}

\begin{table*}[!htp]\centering
	\caption{Impact of customized embedding transformation.}\label{tab:tranformation}
	\scriptsize
				\resizebox{0.9\textwidth}{!}{
	\begin{tabular}{l|llll|llll}\toprule
		\multirow{2}{*}{Embedding Models}&\multicolumn{4}{c}{Retrieval effectiveness} &\multicolumn{4}{c}{Reconstruct effectiveness} \\\cmidrule{2-9}
		&top 10 &top 20 &top 100 &top 1000 &bleu &tf1 &exact &cos \\\midrule
		DPR\_cls &0.748 &0.800 &0.863 &0.914 &70.735 &0.875 &0.319 &0.985 \\
		DPR\_cls\_transform &0.748 &0.800 &0.863 &0.914 &1.178 &0.065 &0.000 &0.443 \\
		\bottomrule
	\end{tabular}
}
\end{table*}


\subsection{Apply vec2text to corpus poisoning attack}

\begin{table*}[!htp]\centering
	\caption{Corpus poisoning results.}\label{tab:poision}
	\scriptsize
	\resizebox{0.9\textwidth}{!}{
		\begin{tabular}{l|l|llll}\toprule
			Attack method &\#  adv. pass. &Recall@10 &Recall@20 &Recall@100 &Recall@1000 \\\midrule
			hotflip &10 &0.006 &0.015 &0.105 &0.532 \\
			vec2text &10 &0.006 &0.012 &0.036 &0.101 \\
			Oracle &10 &0.206 &0.304 &0.575 &0.926 \\\hline
			vec2text &100 &0.061 &0.091 &0.189 &0.401 \\
			Oracle &100 &0.493 &0.620 &0.868 &0.994 \\\hline
			vec2text &1000 &0.268 &0.335 &0.521 &0.791 \\
			Oracle &1000 &0.779 &0.873 &0.980 &1.000 \\
			\bottomrule
		\end{tabular}
	}
\end{table*}



